STIV: Scalable Text and Image Conditioned Video Generation

The field of video generation has made remarkable advancements, yet there remains a pressing need for a clear, systematic recipe that can guide the development of robust and scalable models. In this work, we present a comprehensive study that systematically explores the interplay of model architectures, training recipes, and data curation strategies, culminating in a simple and scalable text-image-conditioned video generation method, named STIV. Our framework integrates image condition into a Diffusion Transformer (DiT) through frame replacement, while incorporating text conditioning via a joint image-text conditional classifier-free guidance. This design enables STIV to perform both text-to-video (T2V) and text-image-to-video (TI2V) tasks simultaneously. Additionally, STIV can be easily extended to various applications, such as video prediction, frame interpolation, multi-view generation, and long video generation, etc. With comprehensive ablation studies on T2I, T2V, and TI2V, STIV demonstrate strong performance, despite its simple design. An 8.7B model with 512 resolution achieves 83.1 on VBench T2V, surpassing both leading open and closed-source models like CogVideoX-5B, Pika, Kling, and Gen-3. The same-sized model also achieves a state-of-the-art result of 90.1 on VBench I2V task at 512 resolution. By providing a transparent and extensible recipe for building cutting-edge video generation models, we aim to empower future research and accelerate progress toward more versatile and reliable video generation solutions.

==> table/mv.tex <==
\begin{table}[t!]
\centering
% \small
\begin{tabular}{l|ccc}
\toprule
\textbf{Model} & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{LPIPS} $\downarrow$ \\
\midrule
% {"psnr": 21.200395881092003, "ssim": 0.7233099077901357, "lpips": 0.14323076669493395}
Zero123++ \cite{shi2023zero123pp} & 21.200 & 0.723 & \textbf{0.143} \\
% {'psnr': 21.643072619767654, 'ssim': 0.7237723646444655, 'lpips': 0.15624068174364408}
STIV-TI2V-XL & \textbf{21.643} & \textbf{0.724} & 0.156 \\
\bottomrule
\end{tabular}
\caption{Multiview generation comparison on GSO \cite{downs2022google}.}
\label{tab:multiview}
\end{table}

==> table/t2v_high_frame_count_initialization.tex <==
\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l|c|c|c|c}
    \Xhline{1pt}
    \multirow{2}{*}{Init.} & \multicolumn{1}{c|}{MSRVTT} & \multicolumn{3}{c}{VBench} \\
    \cline{2-5}
    & FVD $\downarrow$ & Quality $\uparrow$ & Semantic $\uparrow$ & Total $\uparrow$ \\
    \Xhline{1pt}
    T2I                     & 549.13 & 78.71 & 65.69 & 76.10 \\
    T2V (interpolation)           & 407.86 & 79.56 & 65.42 & 76.73 \\
    T2V (extrapolation)           & \textbf{397.90} & 79.18 & 64.63 & 76.27 \\
    T2V 2x (interpolation)        & 401.94 & \textbf{79.59} & \textbf{66.24} & \textbf{76.92} \\
    \Xhline{1pt}
    \end{tabular}
    \caption{Performance of different model initialization methods for higher frame count (40 frames) T2V-XL  model training.}
    \label{tab:t2v_high_frame_count_init}
\end{table}

==> table/t2v_high_res_initialization.tex <==

\begin{table}[h]
    \small
    \centering
    \begin{tabular}{p{1.5cm}|c|c|c|c}
    \Xhline{1pt}
    \multirow{2}{*}{Init.} & \multicolumn{1}{c|}{MSRVTT} & \multicolumn{3}{c}{VBench} \\
    \cline{2-5}
     & FVD $\downarrow$ & Quality $\uparrow$ & Semantic $\uparrow$ & Total $\uparrow$ \\
    \Xhline{1pt}
    Scratch             & 417.98 & 80.27 & 67.84 & 77.78 \\
    T2V-256             & 415.63 & 80.28 & 71.29  & 78.49 \\
    T2I-512             & \textbf{401.83} & 79.77 & 71.58 & 78.13 \\
    Both               & 405.14 & \textbf{80.45} & \textbf{72.37} & \textbf{78.83} \\
    \Xhline{1pt}
    \end{tabular}
    \caption{Performance of different model initialization methods for high resolution (512x512) T2V-XL-512 model training.}
    \label{tab:t2v_high_res_init}
\end{table}

==> table/t2v_modulation.tex <==
% \paragraph{T2V Ablation Studies}
\begin{table}[h!]
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|c|c}
\Xhline{1pt}
\multirow{2}{*}{Module} & \multicolumn{3}{c}{VBench} \\
\cline{2-4}
& Quality $\uparrow$ & Semantic $\uparrow$ & Total $\uparrow$ \\
\Xhline{1pt}
Base model & 80.19 & 70.51 & 78.25 \\
\hspace{1mm} w/ temporal patch=1 & \textbf{80.92} & 71.69 & \textbf{79.07} \\
\hspace{1mm} w/ temporal patch=4 & 79.72 & 69.15 & 77.61 \\
% use CVAE & 80.58 & 73.26 & 79.11 \\
\hspace{1mm} w/ causal temporal\_attention & 74.59 & \textbf{73.13} & 74.30 \\
\hspace{1mm} + temporal scale\_shift\_gate & 80.32 & 68.94 & 78.04 \\
\hspace{1mm} + temporal mask & 77.58 & 65.95 & 75.25 \\
\hspace{1mm} - spatial mask & 80.57 & 70.31 & 78.52 \\
\Xhline{1pt}
\end{tabular}
% }
\caption{Ablation Study of T2V model design using T2V-XL. The base model uses temporal path size 2, non-causal temporal attention, spatial masking ratio 0.5, and no temporal masking.}
\label{tab:modulate_t2v_vbench}
\end{table}

==> table/t2v_videophy.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{l|c|c|c|c}
\Xhline{1pt}
% \multicolumn{5}{|c|}{\textbf{Open Models}} \\ 
\textbf{Model} & \textbf{Source} & \textbf{PC} & \textbf{SA} & \textbf{Avg.} \\
\Xhline{1pt}
OpenSora~\citep{zheng2024open-sora} & Open & 35 & 21 & 28 \\
SVD~\citep{blattmann2023stable} & Open & 34 & 37 & 35 \\
CogVideoX-2B~\citep{yang2024cogvideox} & Open & 39 & 40 & 39 \\
LaVIE~\citep{wang2023lavie} & Open & 36 & 45 & 41 \\
VideoCrafter2~\citep{chen2024videocrafter2}  & Open & 36 & 47 & 41 \\
CogVideoX-5B~\citep{yang2024cogvideox}  & Open & 41 & 57 & 49 \\
\hline
\hline
% \multicolumn{5}{|c|}{\textbf{Closed Models}} \\ \hline
\textbf{Model} & \textbf{Source} & \textbf{PC} & \textbf{SA} & \textbf{Avg.} \\ \Xhline{1pt}
Gen-2~\citep{runway2023gen} & Closed & 31 & 26 & 29 \\
Pika~\citep{pika2023pika} & Closed & 33 & 25 & 29 \\
Lumiere-T2V~\citep{bar2024lumiere} & Closed & 31 & 35 & 33 \\
Lumiere-T2I2V~\citep{bar2024lumiere} & Closed & 25 & 46 & 35 \\
Luma Dream Machine~\citep{luma2024dream}  & Closed & 30 & 53 & 41.5 \\
\hline
XL & Our & 36 & 57 & 47 \\
M-512 & Our & \textbf{43} & \textbf{59} & \textbf{51} \\
\Xhline{1pt}
\end{tabular}
\caption{Performance of T2V models on VideoPhy~\cite{bansal2024videophy}.}
\label{tab:video_phy}
\end{table}

==> table/tup.tex <==
\begin{table}[t!]
\centering
% \small
\begin{tabular}{l|c|cc}
\Xhline{1pt}
\textbf{Model} & \textbf{use text} & \textbf{FID} $\downarrow$ & \textbf{FVD} $\downarrow$ \\
\Xhline{1pt}
STIV-TUP & No & 2.2 & 6.3 \\
STIV-TUP & Yes & 2.0 & 5.9 \\
\Xhline{1pt}
\end{tabular}
\caption{Performance of STIV-TUP on MSRVTT test set.}
\label{tab:t_upsampler_performance}
\end{table}

==> table/tv2v.tex <==
\begin{table}[t!]
% \small
\centering
\begin{tabular}{l|c|c}
\Xhline{1pt}
\textbf{Model} & \textbf{MSRVTT-FVD} $\downarrow$ & \textbf{MovieGen-FVD} $\downarrow$ \\
\Xhline{1pt}
T2V & 536.2 & 347.2 \\
STIV-V2V & 183.7 & 186.3 \\
\Xhline{1pt}
\end{tabular}
\caption{Comparison of FVD scores between text-to-video (T2V) and video-to-video (V2V) models across different datasets.}
\label{tab:tv2v}
\end{table}
